Critical spin chains and loop models with $PSU(n)$ symmetry

Starting with the Ising model, statistical models with global symmetries provide fruitful approaches to interesting physical systems, for example percolation or polymers. These include the $O(n)$ model (symmetry group $O(n)$) and the Potts model (symmetry group $S_Q$). Both models make sense for $n,Q\in \mathbb{C}$ and not just $n,Q\in \mathbb{N}$, and both give rise to a conformal field theory in the critical limit. Here, we study similar models based on the group $PSU(n)$. We focus on the two-dimensional case, where the models can be described either as gases of non-intersecting orientable loops, or as alternating spin chains. This allows us to determine their spectra either by computing a twisted torus partition function, or by studying representations of the walled Brauer algebra. In the critical limit, our models give rise to a CFT that exists for any $n\in\mathbb{C}$ and has a global $PSU(n)$ symmetry. Its spectrum is similar to those of the $O(n)$ and Potts CFTs, but a bit simpler. We conjecture that the $O(n)$ CFT is a $\mathbb{Z}_2$ orbifold of the $PSU(n)$ CFT, where $\mathbb{Z}_2$ acts as complex conjugation.

==> figures/header/macros.tex <==
\makeatletter
\patchcmd{\BR@backref}{\newblock}{\newblock(}{}{}
\patchcmd{\BR@backref}{\par}{)\par}{}{}

\newcommand{\doublewidetilde}[1]{{%
  \mathpalette\double@widetilde{#1}%
}}
\newcommand{\double@widetilde}[2]{%
  \sbox\z@{$\m@th#1\widetilde{#2}$}%
  \ht\z@=.9\ht\z@
  \widetilde{\box\z@}%
}
\makeatother
\newcommand{\aline}{\hspace{1cm}\hfil\rule{0.93\textwidth}{.4pt}}

\numberwithin{equation}{section}
\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}

\newtheoremstyle{break}{9pt}{9pt}{\itshape}{}{\bfseries}{}{\newline}{}
\theoremstyle{break}    
\newtheorem{hyp}{Hypothesis}[section]
\newtheorem{defn}[hyp]{Definition}
\newtheorem{conj}[hyp]{Conjecture}
\newtheorem{thm}[hyp]{Theorem}
\newtheorem{prop}[hyp]{Proposition}

\DeclareMathOperator{\Rep}{Rep\,}
\newcommand{\uline}[1]{%
  \underline{\smash{#1}\vphantom{T}}\vphantom{#1}%
}
\DeclareMathOperator{\Del}{\uline{\mathrm{Rep}}}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Vir}{Vir}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\ind}{ind}
\newcommand{\JTL}{\mathcal{J\!T\!\!L}}



==> figures/header/packages.tex <==
\usepackage[nottoc]{tocbibind}
% For References to appear in the table of contents

\RequirePackage[l2tabu, orthodox]{nag}
\usepackage{silence}
\WarningFilter[pdftoc]{hyperref}{Token not allowed in a PDF string}
\ActivateWarningFilters[pdftoc]

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

% \usepackage{showkeys}

\usepackage[top=20mm, bottom=20mm, left=25mm, right=25mm]{geometry}
% \usepackage{showkeys} % show labels

\usepackage{amsmath, amssymb, amsfonts, amsthm,multirow}
\usepackage{nccmath} % center given equation in fleqn document
\usepackage{bm}  % bold math
\usepackage{array}

\usepackage[colorlinks=true, linktoc=all, linkcolor=black, citecolor=red, urlcolor=blue!50!black, backref=page]{hyperref}
\usepackage{float} %place figures in text

\usepackage{etoolbox}

\usepackage{pgf,pgfplots}
\usepackage{pdflscape,afterpage} %landscape mode
\usepackage{tikz}
\usetikzlibrary{calc, decorations.markings,patterns,arrows,decorations.pathreplacing,shapes.geometric}
\usetikzlibrary{backgrounds,fit,positioning}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
\usepackage{BOONDOX-cal} % Lower-case calligraphic font (and nicer upper case)

\usepackage{tikz-cd}


==> figures/header/tikz_commands.tex <==
%Tikz macros and styles

\tikzset{
midarrow/.style={postaction = decorate, decoration = {markings,
  							 mark = at position 0.6 with {\arrow[scale=2]{stealth}}}}
,upSitearrow/.style={postaction=decorate,decoration={markings,mark=at position 0.7 with {\arrow{angle 60}}}}
,downSitearrow/.style={postaction=decorate,decoration={markings,mark=at position 0.8 with {\arrow{angle 60}}}}
,loops/.style={line width = 3pt, red, rounded corners=6pt, opacity=0.55}
,orientedloops/.style={line width = 3pt, red, rounded corners=6pt, opacity=0.55, postaction=decorate, decoration={markings, mark= at position 0.7 with {\arrow{Stealth}}}}
,uSite/.style={circle,inner sep=0pt}
,dSite/.style={circle,inner sep =0pt}
,thrLine/.style={out=90,in=-90}
,barc/.style={out=90,in=90}
,tarc/.style={out=-90,in=-90}
,wall/.style={black!70!white,dotted}
,site/.style={circle,inner sep=0pt}
,emptysite/.style={circle,radius=3pt,inner sep=0pt}
,orientedbarc/.style={out=90,in=90,postaction=decorate,decoration={markings,mark= at position 0.6 with {\arrow{angle 60}}}}
,orientedtarc/.style={out=-90,in=-90,postaction=decorate,decoration={markings,mark= at position 0.6 with {\arrow{angle 60}}}}
}
%
\newcommand{\CClattice}[2]{
\foreach \i in {0,2,...,#1}{
	\foreach \j in {1,3,...,#2}{
		\draw[midarrow] (\i,\j) -- (\i+1,\j+1);
		\draw[midarrow] (\i+1,\j+1) -- (\i+2,\j);
		\draw[midarrow] (\i+1,\j+1) -- (\i,\j+2);
		\draw[midarrow] (\i+2,\j+2) -- (\i+1,\j+1);
	};};
	\foreach \j in {1,3,...,#2} {
		\draw[midarrow] (-1,\j+1) -- (0,\j);
		\draw[midarrow] (0,\j+2) -- (-1,\j+1);
		\draw[midarrow] (#1+2,\j) -- (#1+3,\j+1);
		\draw[midarrow] (#1+3,\j+1) -- (#1+2,\j+2);
	};
}
%
\newcommand{\uSite}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};%
\draw[upSitearrow] (#1,#2-0.2) -- (#1,#2+0.05);%
}
\newcommand{\dSite}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};%
\draw[downSitearrow] (#1,#2+0.05) -- (#1,#2-0.2);%
}
\newcommand{\site}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};
}
\newcommand{\emptysite}[3]{
\node[emptysite, draw] (#3) at (#1,#2) {};
}

\newcommand{\gol}{ -- ++(-1,0)}
\newcommand{\gor}{ -- ++(1,0)}
\newcommand{\gou}{ -- ++(0,1)}
\newcommand{\god}{ -- ++(0,-1)}

==> header/macros.tex <==
\makeatletter
\patchcmd{\BR@backref}{\newblock}{\newblock(}{}{}
\patchcmd{\BR@backref}{\par}{)\par}{}{}

\newcommand{\doublewidetilde}[1]{{%
  \mathpalette\double@widetilde{#1}%
}}
\newcommand{\double@widetilde}[2]{%
  \sbox\z@{$\m@th#1\widetilde{#2}$}%
  \ht\z@=.9\ht\z@
  \widetilde{\box\z@}%
}
\makeatother
\newcommand{\aline}{\hspace{1cm}\hfil\rule{0.93\textwidth}{.4pt}}

\numberwithin{equation}{section}
\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}

\newtheoremstyle{break}{9pt}{9pt}{\itshape}{}{\bfseries}{}{\newline}{}
\theoremstyle{break}    
\newtheorem{hyp}{Hypothesis}[section]
\newtheorem{defn}[hyp]{Definition}
\newtheorem{conj}[hyp]{Conjecture}
\newtheorem{thm}[hyp]{Theorem}
\newtheorem{prop}[hyp]{Proposition}

\DeclareMathOperator{\Rep}{Rep\,}
\newcommand{\uline}[1]{%
  \underline{\smash{#1}\vphantom{T}}\vphantom{#1}%
}
\DeclareMathOperator{\Del}{\uline{\mathrm{Rep}}}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Vir}{Vir}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\ind}{ind}
\newcommand{\JTL}{\mathcal{J\!T\!\!L}}



==> header/packages.tex <==
\usepackage[nottoc]{tocbibind}
% For References to appear in the table of contents

\RequirePackage[l2tabu, orthodox]{nag}
\usepackage{silence}
\WarningFilter[pdftoc]{hyperref}{Token not allowed in a PDF string}
\ActivateWarningFilters[pdftoc]

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

% \usepackage{showkeys}

\usepackage[top=20mm, bottom=20mm, left=25mm, right=25mm]{geometry}
% \usepackage{showkeys} % show labels

\usepackage{amsmath, amssymb, amsfonts, amsthm,multirow}
\usepackage{nccmath} % center given equation in fleqn document
\usepackage{bm}  % bold math
\usepackage{array}

\usepackage[colorlinks=true, linktoc=all, linkcolor=black, citecolor=red, urlcolor=blue!50!black, backref=page]{hyperref}
\usepackage{float} %place figures in text

\usepackage{etoolbox}

\usepackage{pgf,pgfplots}
\usepackage{pdflscape,afterpage} %landscape mode
\usepackage{tikz}
\usetikzlibrary{calc, decorations.markings,patterns,arrows,decorations.pathreplacing,shapes.geometric}
\usetikzlibrary{backgrounds,fit,positioning}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
\usepackage{BOONDOX-cal} % Lower-case calligraphic font (and nicer upper case)

\usepackage{tikz-cd}


==> header/tikz_commands.tex <==
%Tikz macros and styles

\tikzset{
midarrow/.style={postaction = decorate, decoration = {markings,
  							 mark = at position 0.6 with {\arrow[scale=2]{stealth}}}}
,upSitearrow/.style={postaction=decorate,decoration={markings,mark=at position 0.7 with {\arrow{angle 60}}}}
,downSitearrow/.style={postaction=decorate,decoration={markings,mark=at position 0.8 with {\arrow{angle 60}}}}
,loops/.style={line width = 3pt, red, rounded corners=6pt, opacity=0.55}
,orientedloops/.style={line width = 3pt, red, rounded corners=6pt, opacity=0.55, postaction=decorate, decoration={markings, mark= at position 0.7 with {\arrow{Stealth}}}}
,uSite/.style={circle,inner sep=0pt}
,dSite/.style={circle,inner sep =0pt}
,thrLine/.style={out=90,in=-90}
,barc/.style={out=90,in=90}
,tarc/.style={out=-90,in=-90}
,wall/.style={black!70!white,dotted}
,site/.style={circle,inner sep=0pt}
,emptysite/.style={circle,radius=3pt,inner sep=0pt}
,orientedbarc/.style={out=90,in=90,postaction=decorate,decoration={markings,mark= at position 0.6 with {\arrow{angle 60}}}}
,orientedtarc/.style={out=-90,in=-90,postaction=decorate,decoration={markings,mark= at position 0.6 with {\arrow{angle 60}}}}
}
%
\newcommand{\CClattice}[2]{
\foreach \i in {0,2,...,#1}{
	\foreach \j in {1,3,...,#2}{
		\draw[midarrow] (\i,\j) -- (\i+1,\j+1);
		\draw[midarrow] (\i+1,\j+1) -- (\i+2,\j);
		\draw[midarrow] (\i+1,\j+1) -- (\i,\j+2);
		\draw[midarrow] (\i+2,\j+2) -- (\i+1,\j+1);
	};};
	\foreach \j in {1,3,...,#2} {
		\draw[midarrow] (-1,\j+1) -- (0,\j);
		\draw[midarrow] (0,\j+2) -- (-1,\j+1);
		\draw[midarrow] (#1+2,\j) -- (#1+3,\j+1);
		\draw[midarrow] (#1+3,\j+1) -- (#1+2,\j+2);
	};
}
%
\newcommand{\uSite}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};%
\draw[upSitearrow] (#1,#2-0.2) -- (#1,#2+0.05);%
}
\newcommand{\dSite}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};%
\draw[downSitearrow] (#1,#2+0.05) -- (#1,#2-0.2);%
}
\newcommand{\site}[3]{
\node[circle,inner sep=0pt] (#3) at (#1,#2) {};
}
\newcommand{\emptysite}[3]{
\node[emptysite, draw] (#3) at (#1,#2) {};
}

\newcommand{\gol}{ -- ++(-1,0)}
\newcommand{\gor}{ -- ++(1,0)}
\newcommand{\gou}{ -- ++(0,1)}
\newcommand{\god}{ -- ++(0,-1)}
